On the impact of activation and normalization in obtaining isometric embeddings at initialization

In this paper, we explore the structure of the penultimate Gram matrix in deep neural networks, which contains the pairwise inner products of outputs corresponding to a batch of inputs. In several architectures it has been observed that this Gram matrix becomes degenerate with depth at initialization, which dramatically slows training. Normalization layers, such as batch or layer normalization, play a pivotal role in preventing the rank collapse issue. Despite promising advances, the existing theoretical results do not extend to layer normalization, which is widely used in transformers, and can not quantitatively characterize the role of non-linear activations. To bridge this gap, we prove that layer normalization, in conjunction with activation layers, biases the Gram matrix of a multilayer perceptron towards the identity matrix at an exponential rate with depth at initialization. We quantify this rate using the Hermite expansion of the activation function.

==> abstract.tex <==




%% Version 5
% The kernel function associated with deep neural network outputs has gained attention in both theoretical and practical domains. In simple terms, neural kernels can be viewed as a similarity measure between data points in the transformed space of the last hidden layer. Theoretically, these kernels are critical components of the neural tangent kernel. Experimentally, kernel isometry has been shown to enhance training performance, prompting research on the relationship between neural architectures and kernel isometry. Despite progress, there is still no easy-to-understand explanation of how normalization layers, including batch and layer normalization, influence kernel isometry. Notably, layer normalization, a crucial component in large language models, remains under-explored.

% In this study, we investigate the interactions between normalization, activation and neural kernels. Our findings reveal that normalization layers, including both batch and layer normalization, significantly bias the kernel towards isometry. We introduce the intuitive concept for isometry distance, enabling a Lyapunov analysis on the kernel of infinitely-wide deep neural networks. Using this analysis, we explore the interplay between non-linear activations and layer normalization, uncovering a nuanced connection between the Hermite polynomial expansion of activation functions and kernel isometry. Our analysis highlights the role of coefficients associated with high-order Hermite polynomials in the isometry bias of kernel functions in deep random MLPs with layer normalization.


%% Version 4 %%% 


% The kernel function associated with the output function of deep neural networks has been the subject of theoretical and practical studies. Theoretically, the kernel function is an important component of the neural tangent kernel. In practice, various experimental evidences show that the kernel isometry leads to an enhanced training performance. This motivated research on the interplay of neural architectures on the kernel isometry. Despite the valuable insights and progress in this vein, there is no intuitive sound analysis explaining the impact of various normalization layers ---encompassing batch normalization and layer normalization--- on the kernel isometry. In particular, the role of layer normalization is under-studied, which is an important component of large language models. 


% Towards understanding the interplay of neural architectures with neural kernels, we establish the implicit bias of normalization in the kernel function associated with deep neural networks. We prove the normalization layers, including batch normalization and layer normalization strikingly bias the kernel towards isometry. This isometry bias is formulated using the intuitive notion of isometry gap that allows us to establish a Lyapunov analysis of the kernel associated with deep neural networks in the regime of infinite width. Leveraging this Lyapunov analysis, we analyze the interplay between non-linear activations and layer normalization demonstrating a subtle connection between Hermite polynomial expansion of the activation function and kernel isometry. According to our analysis, activations with large high-order Hermit coefficients impose stronger isometry for the kernel function of deep random MLPs with layer normalization. 

%%% Version 3 %%% 

% The kernel function associated with 
% Various empirical studies highlight the important role of kernel isometry in the optimization of deep neural networks. The components of neural networks, including activation, normalization, and weights shape the kernel with depth. In this paper, we prove the normalization layers, including batch normalization and layer normalization, impose a striking bias towards kernel isometry. This implicit bias allows us to establish a Lyapunov analysis of the kernel associated with deep neural networks in the regime of infinite width. Leveraging this Lyapunov analysis, we analyze the interplay between non-linear activations and layer normalization demonstrating a subtle connection between Hermite polynomial expansion of the activation function and kernel isometry. According to our analysis, activations with zero Hermite coefficient and heavy tail coefficient impose a strong isometry for the kernel function of deep random MLPs with layer normalization. 

%%% Version 2 %%%
% In this study, we present a novel concept of isometry, offering a deeper understanding of the role played by normalisation layers in biasing the neural tangent kernel (NTK) towards isometry. We demonstrate that normalisation layers deterministically improve the isometry of the Gram matrix, which serves as an approximation of the NTK. This finding builds upon and extends previously known stochastic results related to normalisation.
% Furthermore, we reveal that in an MLP with layer normalisation and random weights, the distance to isometry acts as a Lyapunov function for the isometry of Gram matrices across different depths, showing that nonlinear activations bias the kernel in favor of isometry. These findings deliver intuitive explanations for previously observed phenomena, but also shed possibly new light between the differences of batch and layer normalisation. 
% Overall, our novel notion of isometry possesses numerous rich geometric and algebraic properties, which can be harnessed to enhance our theoretical understanding of neural networks and help the development of new modules, such as activation or normalisation layers.


%% Version 1 %%
% This study presents a novel approach for understanding the properties of normalization layers in multilayer perceptrons (MLPs) by introducing isometric gap, a symmetry-preserving metric that measures the deviation from isometry of a covariance or Gram matrix. We explore the behavior of the isometric gap in the context of a normalized MLP, revealing its contractive properties and algebraic features. Our findings indicate that the isometric gap is non-decreasing under normalization and increases when the norms of input rows vary. This insight can be applied to characterize the eigenvalue spectra of MLP representations in depth, helping to advance our understanding of deep learning networks and their behavior.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\appendix




==> defs.tex <==
\usepackage{lipsum}                     % Dummytext
\usepackage{xargs}
\usepackage{xfrac}
\usepackage{amssymb}
\usepackage{amsmath}


\usepackage{mathtools}
\usepackage{algorithm2e}
\usepackage{dsfont}
\newcommand {\bn}{\text{BN}}
\newcommand{\qsim}{\stackrel{\alpha,\beta}{\sim}}
\newcommand{\rank}{{\text{rank}}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\cov}[2]{\text{Cov}\left[#1, #2\right]}
\newcommand{\Ex}[1]{\E\left[#1\right]}
\newcommand{\dw}{\nabla_{\w}}
\newcommand{\tv}{\Tilde{\v}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\sign}{\text{sign}}
\newcommand{\sqnorm}[1]{\left\|#1\right\|^2} 
\newcommand{\tr}{\text{Tr}}
\newcommand{\vectornorm}[1]{\left\|#1\right\|}
\newcommand{\norm}[1]{{}\left\| #1 \right\|}
\newcommand\iid{i.i.d. }

% Vectors
\newcommand{\ip}[2]{\langle #1,#2\rangle}
\newcommand{\Normal}{\mathcal{N}}
\def\1{\mathds{1}}
\newcommand{\ReLU}{F^{+}}
\newcommand\distas{\stackrel{\mathrm{dist.}}{=}}
\newcommand{\law}{\mathrm{law}}
\newcommand\Abs{\mathrm{abs}}
\newcommand{\Fourier}{\mathcal{F}}
\newcommand{\iFourier}{\mathcal{F}^{-1}}
\newcommand\sgn{\mathrm{sgn}}
\newcommand{\gf}{\nabla f}
\newcommand{\gft}{{\nabla \tilde{f}}}
\newcommand{\hf}{\nabla^2 f} % Hessian
\newcommand{\av}{{\bf a}}
\newcommand{\as}{{\mathcal A}}
\newcommand{\bs}{{\mathcal B}}
\newcommand{\var}{{\bf var}}
\newcommand{\g}{{\bf g}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\gb}{\bar{g}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\s}{{\bf s}}
\newcommand{\shat}{\hat{s}}
\newcommand{\w}{{\bf w}}
\renewcommand{\u}{{\bf u}}
\renewcommand{\d}{{\bf d}}
\newcommand{\pw}{\tilde{\w}}
\newcommand{\we}{\tilde{\w}}
\newcommand{\wstar}{\w^*}
\newcommand{\wtil}{{\tilde{\bf w}}}
\newcommand{\x}{{\bf x}}
\renewcommand{\a}{{\bf a}}
\newcommand{\blambda}{\boldsymbol{ \lambda}}
\newcommand{\K}{{\bf K}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\X}{{\bf X}}
\newcommand{\y}{{\bf y}}
\newcommand{\Y}{{\bf Y}}
\renewcommand{\v}{{\bf v}}
\newcommand{\z}{{\bf z}}
\newcommand{\q}{{\bf q}}

\newcommand{\eb}{{\bf e}}
\newcommand{\evec}{{\bf e}}
\newcommand{\supervector}{{\bf v}}
\newcommand{\V}{{\cal V}}
\renewcommand{\rm}{{\mathcal R}}
\renewcommand{\S}{{\mathcal S}}
\newcommand{\vb}{{\bf v}}
\newcommand{\pim}{\boldsymbol{\pi}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\tbigo}{\tilde{{\cal O}}}
\usepackage{amsmath,amssymb}
\renewcommand{\Ex}{\mathbb{E}}
% Matrices
\def\Am{{\bf A}}
\def\Bm{{\bf B}}
\def\Hm{{\bf H}}
\def\Qm{{\bf Q}}
\def\Im{{\bf I}}
\def\T{{\mathcal T}}
\def\Zm{{\bf Z}}
\def\Ym{{\bf Y}}
\def\Xm{{\bf X}}
\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
\newcommand{\M}{{\bf M}}

%\newcommand{\Gamma}{{\bf \gamma}}
\newcommand{\U}{{\bf U}}
\renewcommand{\V}{{\bf V}}
\newcommand{\D}{{\bf D}}
\renewcommand{\cov}{{\bf S}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\zero}{{\bf 0}}
\newcommand{\ones}{{\bf 1}}
\newcommand{\C}{{\bf C}}

\newcommand{\W}{{\mathcal W}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\Efull}{\mathbb{E}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\expd}{{\mathcal Exp}}
\newcommand{\Z}{{\mathbf Z}}
\newcommand{\J}{{\mathbf J}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\ve}{\text{v}}
\newcommand{\Q}{{\mathcal Q}}
\newcommand{\Event}{{\mathcal E}}
\newcommand{\row}{{\mathrm{row}}}
\renewcommand{\tv}[2]{\norm{\mu_{#1}-\mu_{#2}}_{tv}}
\renewcommand{\C}{{G_*}}
\renewcommand{\S}{{\mathcal S}}
\newcommand{\BN}{{\phi}}
\renewcommand{\F}{{\sigma}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\V}{\mathcal{V}}
\newcommand{\I}{{\mathbf I}}
\newcommand{\gap}{\text{gap}}
\renewcommand{\P}{{\mathcal P}}
\renewcommand{\Pr}{{\mathbb{P}}}
\newcommand{\indic}{\mathbbm{1}} 
\newcommand{\cosa}[3]{\cos \angle_{#1} (#2,#3)}
\newcommand{\sina}[3]{\sin \angle_{#1} (#2,#3)}
\newcommand{\cosapow}[4]{\cos^{#1} \angle_{#2} (#3,#4)}
\newcommand{\sinapow}[4]{\sin^{#1} \angle_{#2} (#3,#4)}
\newcommand{\cosasq}[3]{\cos^2 \angle_{#1} (#2,#3)}
\newcommand{\sinasq}[3]{\sin^2 \angle_{#1} (#2,#3)}

\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\diag}{\text{diag}}
\newcommand{\gt}{g_{\text{thres}}}
\newcommand{\e}{\mathbf{e}}
\renewcommand{\rq}{\rho}
\newcommand{\fls}{f_{\text{{\sc ls}}}}
\newcommand{\flh}{f_{\text{{\sc lh}}}}
\newcommand{\fnn}{f_{\text{{\sc nn}}}}
\newcommand{\tn}{t_{\text{noise}}}
\newcommand{\kt}{k_{\text{thres}}}
\newcommand{\kur}{\text{kur}}
\newcommand{\tdir}{T_{\text{d}}}
\newcommand{\tgd}{T_{\text{gd}}}
\newcommand{\tsc}{T_{\text{s}}}
\newcommand{\INDSTATE}[1]{\STATE \hspace{2mm} #1}

\newcommand{\al}[1]{{\color{blue}{#1}}}
\newcommand{\bri}[1]{{\color{red}{#1}}}
\newcommand{\avg}{\text{avg}}


\usepackage{mdframed}
\usepackage{algorithmicx}


\newcommand{\highlight}[1]{\textcolor{red}{#1}}
\usepackage{eqparbox}
\newcommand{\comment}[1]{}

\usepackage{amsthm}


\newtheorem{assumption}{Assumption}
\newtheorem*{assumption*}{\assumptionnumber}
\providecommand{\assumptionnumber}{}
\makeatletter
\newenvironment{assumptioncost}[2]
 {%
  \renewcommand{\assumptionnumber}{Assumption $\mathcal{A}_#1(#2)$}%
  \begin{assumption*}%
  \protected@edef\@currentlabel{$\mathcal{A}_#1$}%
 }
 {%
  \end{assumption*}
 }
 \makeatother

\usepackage{thmtools,thm-restate}




\usepackage{eqparbox}
